HERO: Human-Feedback Efficient Reinforcement Learning for Online Diffusion Model Finetuning

Controllable generation through Stable Diffusion (SD) fine-tuning aims to improve fidelity, safety, and alignment with human guidance. Existing reinforcement learning from human feedback methods usually rely on predefined heuristic reward functions or pretrained reward models built on large-scale datasets, limiting their applicability to scenarios where collecting such data is costly or difficult. To effectively and efficiently utilize human feedback, we develop a framework, HERO, which leverages online human feedback collected on the fly during model learning. Specifically, HERO features two key mechanisms: (1) Feedback-Aligned Representation Learning, an online training method that captures human feedback and provides informative learning signals for fine-tuning, and (2) Feedback-Guided Image Generation, which involves generating images from SD's refined initialization samples, enabling faster convergence towards the evaluator's intent. We demonstrate that HERO is 4x more efficient in online feedback for body part anomaly correction compared to the best existing method. Additionally, experiments show that HERO can effectively handle tasks like reasoning, counting, personalization, and reducing NSFW content with only 0.5K online feedback. The code and project page are available at https://hero-dm.github.io/.

==> content_tex/alg.tex <==
\begin{algorithm}[H]
            \caption{\myshorttitle{}'s Training}\label{alg}
            \begin{algorithmic}[1]
                \Require pretrained SD weights $\phi$, best image ratio $\beta$, feedback budget $N_{\text{fb}}$
                \Initialize learnable weights $\theta$,
                % learnable weights $\theta$ for $E_{\theta}$ and $g_{\theta}$,
                number of feedback $n_{\text{fb}} = 0$, latent distribution $\pi_{\text{HERO}} = \mathcal{N}(\mathbf{0}, \mathbf{I})$
                \While {$n_{\text{fb}} < N_{\text{fb}}$}
                    \State{Sample $n_{\text{batch}}$ noise latents $\rvz_T$ from  $\pi_{\text{HERO}}$}
                    \State{Perform denoising process for each $\rvz_T$ to obtain trajectory $\{\rvz_T, \rvz_{T-1},\cdots, \rvz_0\} $}.
                    \State{Decode $\mathcal{Z}_0$ with SD decoder for images $\mathcal{X}$.}
                    % \State{Sample $n_{\text{batch}}$ images $\displaystyle \mathcal{X}$ from $\phi$ using noise latents $\rvz \sim p_T$}
                    \State{Query human feedback on $\displaystyle \mathcal{X}$, and save corresponding $\displaystyle \mathcal{Z}^+_T$, $\mathcal{Z}^-_T$,  $\rvz^{\text{best}}_T$ }.
                    \State{$n_{\text{fb}} \mathrel{+}= n_{\text{batch}}$}.
                    \State{Update ${\theta}$ of  $E_{\theta}$ and $g_{\theta}$ by minimizing Eq.~\eqref{eqn:encoder-loss}}.
                    \State{Compute reward $R(\rvz_0)$ according to Eq.~\eqref{eqn:reward}}.
                    \State{Update $\phi$ via DDPO by minimizing Eq.~\eqref{eqn:DDPO-K-loss}}.
                    \State{Update latents distribution $\pi_{\text{HERO}}$ using Eq.~\eqref{eqn:sampling}}.
                    % \State Sample {$\displaystyle \mathcal{X}$ from $\phi$ using noise latents chosen from $\displaystyle \mathcal{X}^+$ and $x^{\text{best}}$ according to $\beta$}
                \EndWhile
            \end{algorithmic}
        \end{algorithm}


%  \begin{wrapfigure}{r}{0.65\textwidth}
%       \begin{minipage}{0.6\textwidth}
%         \begin{algorithm}[H]
%             \caption{\myshorttitle{}'s Training}\label{alg}
%             \begin{algorithmic}[1]
%                 \Require pretrained SD weights $\phi$, best image ratio $\beta$, feedback budget $N_{\text{fb}}$
%                 \Initialize learnable weights $\theta$,
%                 % learnable weights $\theta$ for $E_{\theta}$ and $g_{\theta}$,
%                 number of feedback $n_{\text{fb}} = 0$, latent distribution $\pi_{\text{HERO}} = \mathcal{N}(\mathbf{0}, \mathbf{I})$
%                 \While {$n_{\text{fb}} < N_{\text{fb}}$}
%                     \State{Sample $n_{\text{batch}}$ noise latents $\rvz_T$ from  $\pi_{\text{HERO}}$}
%                     \State{Perform denoising process for each $\rvz_T$ to obtain trajectory $\{\rvz_T, \rvz_{T-1},\cdots, \rvz_0\} $}.
%                     \State{Decode $\mathcal{Z}_0$ with SD decoder for images $\mathcal{X}$.}
%                     % \State{Sample $n_{\text{batch}}$ images $\displaystyle \mathcal{X}$ from $\phi$ using noise latents $\rvz \sim p_T$}
%                     \State{Query human feedback on $\displaystyle \mathcal{X}$, and save corresponding $\displaystyle \mathcal{Z}^+_T$, $\mathcal{Z}^-_T$,  $\rvz^{\text{best}}_T$ }.
%                     \State{$n_{\text{fb}} \mathrel{+}= n_{\text{batch}}$}.
%                     \State{Update ${\theta}$ of  $E_{\theta}$ and $g_{\theta}$ by minimizing Eq.~\eqref{eqn:encoder-loss}}.
%                     \State{Compute reward $R(\rvz_0)$ according to Eq.~\eqref{eqn:reward}}.
%                     \State{Update $\phi$ via DDPO by minimizing Eq.~\eqref{eqn:DDPO-K-loss}}.
%                     \State{Update latents distribution $\pi_{\text{HERO}}$ using Eq.~\eqref{eqn:sampling}}.
%                     % \State Sample {$\displaystyle \mathcal{X}$ from $\phi$ using noise latents chosen from $\displaystyle \mathcal{X}^+$ and $x^{\text{best}}$ according to $\beta$}
%                 \EndWhile
%             \end{algorithmic}
%         \end{algorithm}
%     \end{minipage}
% \end{wrapfigure}
    

==> text/backup/1_intro_backup.tex <==
\section{Introduction}


\begin{figure}[h]
    \begin{center}
        \includegraphics[width=0.8\textwidth]{figures/overview_v9.png}
    \end{center}
    \caption{\textbf{\textcircled{0} Online Human Feedback on Generated Images:} Each epoch, SD generates a batch of images, evaluated by a human as ``good'' or ``bad'', with the ``best'' among the ``good'' selected. The corresponding SD noises and latents are saved.
\textbf{\textcircled{1} Learning Human-Aligned Representations:} Human-annotated images train an embedding map via contrastive learning, converting feedback into continuous representations. These are rated by cosine similarity to one of the ``best'' images and used to fine-tune SD via DDPO~\citep{black2024trainingdiffusionmodelsreinforcement}.
\textbf{\textcircled{2} Generating New Images from Refined Noises:} New images are generated from a Gaussian mixture centered around the recorded noises of ``good'' images. This process is repeated until the feedback budget is exhausted.} 
    \label{fig:overview}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Human-controllable \sun{"human" seems redundant} text-to-image (T2I) generation focuses on aligning model outputs with human \sun{maybe "user"?} intent, such as producing realistic images (e.g., undistorted human bodies) or accurately reasoning \sun{how is this reasoning?} about count, semantics, or attributes. A common approach involves fine-tuning latent diffusion models (DM) like Stable Diffusion (SD)~\citep{rombach2022high} using reinforcement learning (RL)-based methods~\citep{winata2024preference}. However, much of the prior works~\citep{fan2023dpokreinforcementlearningfinetuning,black2024trainingdiffusionmodelsreinforcement,rafailov2024directpreferenceoptimizationlanguage,wallace2023diffusionmodelalignmentusing} depend on task-specific, large-scale \emph{offline} human-labeled datasets or pretrained models built on these datasets, which are costly and difficult to collect. For example, \cite{black2024trainingdiffusionmodelsreinforcement} utilizes the LAION aesthetics dataset with 176K human image ratings~\citep{schuhmann2022laion} to enhance aesthetic quality, while \cite{wallace2023diffusionmodelalignmentusing} leverages the Pick-a-Pic dataset~\citep{kirstain2023pick} with 851K pairwise human preferences for T2I alignment. 
Additionally, this offline crowdsourced dataset may raise copyright or legal concerns~\citep{birhane2024into}, and lead to further laborious filtering efforts on top of data collection.

Recently, D3PO~\citep{yang2024using} introduces an alternative method that leverages \emph{online} human feedback for fine-tuning diffusion models (DMs). By collecting feedback during training for specific tasks, this approach enables task-specific solutions, such as correcting distorted human bodies, without requiring large offline datasets. However, it still necessitates approximately 5K instances of online human feedback during training~\citep{yang2024using, uehara2024feedbackefficientonlinefinetuning}. Overall, the practicality of current methods remains constrained by their reliance on extensive human feedback (whether offline or online), highlighting the need for more feedback-efficient approaches.



In this work, we propose \textbf{HERO}—Human-feedback Efficient Reinforcement learning for Online diffusion model fine-tuning—to effectively utilize \emph{online} human feedback while minimizing the need for large-scale queries. As illustrated in Fig.~\ref{fig:overview}, at each epoch, SD generates a batch of images, a human evaluator classifies the images as ``good'' or ``bad'', selecting one ``best'' image from the ``good'' set, and their corresponding SD latents and noise used in image generation are stored. The latents of the human-annotated images are then employed to train an embedding map through contrastive learning~\citep{chen2020simpleframeworkcontrastivelearning}, aiming to develop a human-aligned representation space. By calculating the cosine similarity to the ``best'' representation vector in the learned representation space, we obtain a continuous evaluation for each latent, allowing us to derive a gradation among all ``good'' or ``bad'' latents. Subsequently, we apply Denoising Diffusion Policy Optimization (DDPO)~\citep{black2024trainingdiffusionmodelsreinforcement}, utilizing the computed similarity as continuous reward signals to fine-tune SD via LoRA~\citep{hu2021lora}. 
\input{content_tex/teaser_fig} 
In the next epoch, we sample new batch of images from a Gaussian mixture centered on the stored ``good'' and ``best'' initial noises from the previous iteration. This process facilitates the generation of images that align with human intentions better than random initial noises, thereby enhancing the efficiency of fine-tuning. The above processes—embedding learning for extracting meaningful representations for DDPO fine-tuning and refining initial noises for generation—are repeated until the feedback budget is reached.
% \djk{Does the final sentence make sense?}

At a high level, \myshorttitle{} contains two novel components: (1) \emph{Learning Human-Aligned Representations}, an online-trained embedding map that creates a representation space that implicitly captures human preferences and provides continuous reward signals for RL fine-tuning, and (2) \emph{Generating from Refined Initial Noises}, which involve generating images from SD's refined initialization samples aligned with human intent, for faster convergence to the evaluator's preferences.
These innovations enable \myshorttitle{} to achieve rapid convergence to individual evaluator preferences, significantly reducing the amount of required human feedback. Additionally, \myshorttitle{} effectively tackles challenging tasks that demand conceptual reasoning, such as generating non-deformed objects with specified counts, colors, and contexts—tasks where previous methods, including prompt enhancement~\citep{winata2024preference} and fine-tuning approaches that rely on a few reference images~\citep{gal2022imageworthwordpersonalizing, ruiz2023dreambooth}, have struggled (see illustration in Fig.~\ref{fig:hand-comparison} and more results in Sec.~\ref{sec: experiments}).  
We summarize the features and contributions of \myshorttitle{} as follows: 
\begin{itemize} 
    \item \myshorttitle{} significantly reduces the amount of \emph{online} human feedback required for RL fine-tuning of SD. Our approach typically requires only 0.5K-1K online feedback, decreasing the requirement by at least fourfold compared to the D3PO baseline. This is achieved through two novel features: (1) learning human-aligned representations; (2) sampling from refined initial noises. 
    \item We comprehensively demonstrate the efficacy of \myshorttitle{} across various scenarios, including personalization, complex tasks such as conceptual generation and correction of deteriorated outputs, and NSFW content prevention.
\end{itemize}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Version 1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \cyan{Human-controllable generation in text-to-image (T2I) latent diffusion models, such as Stable Diffusion (SD)~\citep{rombach2022high}, aims to align model outputs more closely with human intent. 
% While fine-tuning diffusion models (DMs)~\citep{hu2021lora, ruiz2023dreambooth, mokady2023null} is an effective approach, fine-tuned models still struggle in tasks that require conceptual reasoning (e.g., generating non-deformed objects with specified count, color, and context), even with advanced prompt engineering (see Fig.~\ref{fig:hand-comparison}). \ayano{aim to improve clarity; update to match the new fig 1 better}
% Reinforcement learning (RL)-based finetuning approaches have emerged, but most prior works~\citep{fan2023dpokreinforcementlearningfinetuning,black2024trainingdiffusionmodelsreinforcement,rafailov2024directpreferenceoptimizationlanguage,wallace2023diffusionmodelalignmentusing} depend on large-scale offline human-labeled datasets or pre-trained models built on these datasets, which are often task-specific and lack coverage of diverse tasks or modalities.

% Human-controllable text-to-image (T2I) generation aims to align model outputs more closely with human intent. A common approach is fine-tuning latent diffusion models, such as Stable Diffusion (SD)~\citep{rombach2022high}.
% Although existing methods have been successful, their performance is highly dependent on the amount of data used for fine-tuning.
% \sfc{explicitly point out data requirement}
% For instance, methods that do not require training images, \ie prompt engineering \todo{refs for prompt enhancement?}, or require only a few reference images~\citep{gal2022imageworthwordpersonalizing, ruiz2023dreambooth} struggle in tasks that require conceptual reasoning (e.g., generating non-deformed objects with a specified count, color, and context).(see Fig.~\ref{fig:hand-comparison}).
% \todo{using more data for DB has not been discussed yet}

% \violet{Reinforcement learning (RL)-based finetuning approaches~\citep{fan2023dpokreinforcementlearningfinetuning,black2024trainingdiffusionmodelsreinforcement,rafailov2024directpreferenceoptimizationlanguage,wallace2023diffusionmodelalignmentusing} provide solutions of using large-scale datasets or pretrained models built on these datasets for challenging tasks, such as aesthetic quality enhancement and text-to-image alignment.
% However, the data requirement is extensive— \cite{black2024trainingdiffusionmodelsreinforcement} uses the LAION aesthetics dataset with 176K human image ratings~\citep{schuhmann2022laion} to enhance aesthetic quality, while \cite{wallace2023diffusionmodelalignmentusing} utilizes the Pick-a-Pic dataset~\citep{kirstain2023pick} with 851K pairwise human preferences for text-to-image alignment.
% In addition, large-scale datasets are not only challenging to collect but can also raise copyright and legal concerns when crowdsourced~\citep{birhane2024into}, making their use for other specific tasks, \eg conceptual reasoning, even more complicated.}


% % Recently, D3PO~\citep{yang2024using} offers an alternative by using online human feedback to fine-tune diffusion models for complex tasks, like correcting distorted human bodies, without the need for large offline datasets.
% % However, it still requires nearly 5K feedback instances during training~\citep{yang2024using, uehara2024feedbackefficientonlinefinetuning}. 
% \violet{Recently, D3PO~\citep{yang2024using} offers an alternative by using online human feedback to fine-tune diffusion models.
% Given the feedback collected during training for individual tasks, D3PO can resolve distorted human body correction without the need for large offline datasets.}
% However, it still requires nearly 5K online human feedback instances during training~\citep{yang2024using, uehara2024feedbackefficientonlinefinetuning}.
% % Overall, existing methods rely heavily on large amounts of human feedback (offline or online), which restricts their practicality. Thus, more human-feedback-efficient methods are needed.
% \cyan{Overall, the practicality of existing methods is limited due to their reliance on large-scale human feedback data (offline or online), calling for a more human-feedback-efficient method.} \ayano{combine 2 sentences}
% % \djk{what's the take-away in this paragraph? I think the reader should infer the author's intention. Could be better to make the take-away more direct.}

% In this work, we propose {\color{cyan}\textbf{HERO}}—{\color{cyan}\textbf{H}}uman-feedback {\color{cyan}\textbf{E}}fficient {\color{cyan}\textbf{R}}einforcement learning for {\color{cyan}\textbf{O}}nline diffusion model fine-tuning—to efficiently utilize \emph{online} human feedback and reduce the need for large-scale queries. Fig.~\ref{fig:overview} shows the pipeline: At each epoch, SD generates around 0.1K images, which a human evaluator categorizes as ``good'' or ``bad'', selecting one ``best'' image from the ``good'' ones. The noise samples used to generate these images are recorded. Human-annotated images are then used to train an \violet{embedding map} with contrastive learning~\citep{chen2020simpleframeworkcontrastivelearning} to learn a human-aligned representation space. 
% \violet{By calculating the cosine similarity to the ``best'' latent, we can obtain a continuous evaluation for each latent and derive a gradation among all ``good'' or ``bad'' latents.} \sfc{give high-level intuition on why this can help improve the efficiency}
% \violet{Then, we apply Denoising Diffusion Policy Optimization (DDPO)~\citep{black2024trainingdiffusionmodelsreinforcement} using the similarity computed above as reward signals to fine-tune SD via LoRA~\citep{hu2021lora}.}\sfc{Define DDPO}
% % These representationsDenoising Diffusion Policy Optimization (DDPO) are scored based on their cosine similarity to the ``best'' image, and the similarity scores serve as the reward signals in DDPO to fine-tune SD via LoRA~\citep{hu2021lora}. 

% % In the next round, new images are sampled from a Gaussian mixture using the recorded noise from ``good'' and ``best'' images.
% \violet{In the next round, we leverage the human selection from the last iteration and sample new images from a Gaussian mixture centered on the stored ``good'' and ``best'' noises. This can help SD generate images that match the human intention and, therefore, improve the efficiency of finetuning.}\sfc{give high-level intuition on why this can help improve the efficiency}
% \violet{The above representation learning and conditioned image generation processes repeat until the evaluator is satisfied.} \sfc{Specify what processes repeat}


% \myshorttitle{} achieves rapid convergence toward the individual evaluator preferences, significantly reducing the amount of human feedback needed while preventing mode collapse. \sfc{we did not explicitly discuss mode collapse above. Maybe remove this?}
% We summarize the features and contributions of \myshorttitle{} as follows: 
% \begin{itemize} 
%     \item \myshorttitle{} is an efficient online human feedback algorithm for fine-tuning SD, enabling personalized, controllable generation without the need for large-scale pre-collected annotated data. 
%     % It reduces online feedback by at least 75\% compared to the baseline D3PO, typically requiring just 0.5K-1K feedback instances in total.
%     \cyan{Typically requiring only 0.5k-1k feedback, \myshorttitle{} reduces online feedback requirement by at least 4 times compared to the D3PO baseline.} \ayano{reorganize and change "75\%" to "4 times"}
%     % \sfc{when comparing to D3PO (hand), we use 1152 samples}
%     % \item We comprehensively show \myshorttitle{}'s efficacy in various scenarios, including personalization and preventing NSFW content, as well as in challenging tasks like conceptual generation and correcting deteriorated outputs.
%     \item \cyan{We comprehensively show \myshorttitle{}'s efficacy in various scenarios, including personalization and NSFW content prevention, as well as in challenging tasks like conceptual generation and correction of deteriorated outputs.}
%     % \sfc{Do we want to claim transferability as part of our contribution? I am not sure...}
%     % Interestingly, finetuned SD with \myshorttitle{} may exhibit some transferability. Specifically, the recorded noise from selected good images and \myshorttitle{}'s finetuned SD on an evaluator's preferred concept (e.g., training prompt \prompt{sexy}, with less nudity favored) can be applied to a different concept (e.g., with other unsafe prompts during testing, the generated images from the finetuned SD and stored noise SD latents contain fewer NSFW images).
% \end{itemize}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{wrapfigure}{r}{0.5\textwidth}
  
%     \includegraphics[width=0.48\textwidth]{birds}
%   \end{center}
%   \caption{Birds}
% \end{wrapfigure}


% \jcc{General Comments on Notations:
% \begin{itemize}
%     \item Categorize notations into three classes:
%         \begin{enumerate}
%             \item Using \texttt{\textbackslash mathcal} mode to represent image "set". For instance, $\mathcal{X}$, $\mathcal{Z}$ mean the image sets and the corresponding SD's encoded latent.
%             \item Using \texttt{\textbackslash mathbf} (or \texttt{\textbackslash rv[character]} mode to represnet sample (it is a vector), such as $\rvx$, $\rvz$, $\rvc$
%             \item Using pure english letter to represent functions, such as $g(\cdot)$, $H(\cdot)$. If we want to write something fancy, we can use \texttt{\textbackslash mathscr}. Such as our feedback encoder $\mathscr{E}(\cdot)$
%         \end{enumerate}
%     \item About subscript or super-script
%     \begin{itemize}
%         \item Preventing using single letter to abbreviate some descriptive contents in subscript or super-script. Such as do not use ``p'' to represent ``postive'', or ``n'' to represent ``negative''. Try to use some descriptive abbreviation in subscript or super-script, such as $\rvx_{\text{best}}$, $\rvx_{\text{pos}}$, $\rvx_{\text{neg}}$
%         \item Using \texttt{\textbackslash text} mode to wrap the descriptive subscript or super-script
%         \item Minor stuff: we can use subscript $t$ in $\rvx_t$ to generally represent time-dependent sample in DM and use super-script $\rvx_t^{(i)}$ if we want to indicate the sample in a batch.
%     \end{itemize}
    
% \end{itemize}
% }


% \jcc{General Comments on Notations:
% \begin{itemize}
%     \item Categorize notations into four classes:
%         \begin{enumerate}
%             \item \textbf{Vector:} Using \texttt{\textbackslash mathbf} (or \texttt{\textbackslash bm{[character]}} mode to represnet sample (it is a vector), such as $\mathbf{X}$, $\bm{y}$; or vector valued function $\bm{f}(\cdot)$
%             \item \textbf{Function:} Using pure english letter to represent functions, such as $g(\cdot)$, $f(\cdot)$. 
%             \item \textbf{Linear function:} For matrix (or linear operator), do we use pure capitalized english letter? Such as the linear corruption kernel $A$ and identity matrix $I_{m\times m}$??
%             \item \textbf{Fancier function or losses:} If we want to write something fancy, we can use \texttt{\textbackslash mathscr} or \texttt{\textbackslash mathcal}. For instance, the corruption kernel $\mathcal A$? For different losses or diveregence, such as, shall we use $\mathcal D_{\text{KL}}$, $\mathcal{J}_{\text{DSM}}$
%         \end{enumerate}
%     \item About NN's parameters, do we use Greek alphabet without \textbf{bold}? Such as $\theta$, $\varphi$ instead of $\bm{\theta}$ and $\bm{\varphi}$??
%     \item About subscript or super-script
%     \begin{itemize}
%         \item Using \texttt{\textbackslash text} mode to wrap the descriptive subscript or super-script
%     \end{itemize}
    
% \end{itemize}
% }


%%% Ayano's Outlines for the Introduction %%%
% \todo{}
%     Build up the motivation for our method, referencing relevant related works.
%     \begin{enumerate}
%         \item Improving text-to-image diffusion models' ability to generate high-fidelity and safe images that align better with human intentions has been a popular problem of interest. One way to achieve this is through diffusion model fine-tuning.
%         \begin{itemize}
%             \item Introduce RL-based diffusion model fine-tuning methods : DDPO, DPOK, SEIKO?, DRaFT
%             \item DPO and Diffusion-DPO
%             \item mention that these are two main methods, and we decide to pursue the RL method
%         \end{itemize}
%         \item DreamBooth
%         \begin{itemize}
%             \item DB is a method that uses human input other than feedback (images) to fine-tune diffusion models
%             \item It is powerful and efficient but its strength is in personalization, and struggles in some challenging tasks like hand anomaly correction
%         \end{itemize}
%         \item Motivate online human feedback by referencing D3PO and DPOK
%         \begin{itemize}
%             \item Most prior methods use large-scale offline datasets for training (expensive to collect, and existing datasets cannot necessarily cover a task of interest)
%             \item Reference DPOK - showed online RL over supervised training on offline data
%             \item D3PO demonstrated that online human feedback is a powerful tool in fine-tuning diffusion models for challenging tasks while avoiding the problems with large-scale offline data
%             \item Weakness : human feedback requirement is very high, calling for a method that is more human-feedback-efficient
%             \item Potentially : One way to reduce human feedback requirement is active query, but this often require a separate network to predict human feedback or a method to estimate the value of queries, which can be challenging, given a limited number of human feedback? To avoid this, we focus on "how to use the feedback more effectively" rather than "how to ask for the most effective feedback"
%         \end{itemize}
%         \item Online human feedback is promising, but to combine this with RL, the question is what sort of feedback to use and how to convert the feedback into rewards
%         \begin{itemize}
%             \item One common way is to train a model that predict human feedback, and use this prediction model as reward for RL training, but this has high data requirement - cite papers listed in representation learning section
%             \item To minimize the human evaluator effort, we choose binary feedback, and avoid the challenges of training a reward model by using human feedback for representation learning instead
%         \end{itemize}
%         \item Highlight our method's applicability to various tasks by mentioning that many prior works focus on specific subset of tasks
%         \begin{itemize}
%             \item Reasoning : Reduce Reuse Recycle, ConceptBed, CDD-ICM, SUR-adapter?
%             \item emotion transfer : Emo-Gen
%             \item personalization : DB, TI
%             \item Text-to-image alignment?
%             \item Safety, hand generation, etc.
%         \end{itemize}
%         \item Contribution : online RLHF algorithm for diffusion model fine-tuning with the following features
%             \begin{itemize}
%                 \item Human-feedback-efficient training achieved by (1) using feedback for representation learning rather than reward learning, and (2) using noise latents of human-selected images for next batch image generation
%                 \item Applicability to variety of tasks, including those challenging for existing methods (e.g. hand anomaly correction)
%                 \item Ability to improve task success and capture personal preferences simultaneously
%             \end{itemize}
%         \item Mention that we also observe transferability of certain personal preferences and concepts to related tasks (not main feature)
%     \end{enumerate}

    %%% Already included in the introduction --> skip 
    % With advancements in AI, text-to-image (T2I) diffusion models has become a widespread tool familiar to many \todo{potentially mention some common models like Stable Diffusion, DALL-E?}. Naturally, expanding T2I models' abilities in generating high-fidelity, safe, and diverse images that align with human intentions, is a major problem of interest today, and there has been a number of works that acheive improvement through T2I model finetuning. 

    %%% Already included in the introduction section --> skip
    % \textit{\textbf{\methodFull}.} 
    % Aforementioned works in T2I diffusion model finetuning has high data requirements, and many are focused on a specific category of tasks. In light of this, we present an online reinforcement learning from human feedback (RLHF) framework for diffusion model finetuning \methodFull (\method). Our main contributions are as follows:
    % \begin{enumerate}
    %     \item \textbf{Human-fedback-efficient training} achieved by (1) utilizing human labels for learning representations that capture human feedback and (2) leveraging noise latents that generated human-favored images for sampling.
    %     \item Applicability to a \textbf{variety of tasks} including deformation correction, content safety improvement, reasoning, and personalization.
    %     \item Ability to achieve \textbf{task success} and \textbf{personal preference alignment} simultaneously.
    % \end{enumerate}
    % In addition to the above, we observe an auxillary capability to transfer certain concepts and preferences to related tasks, although performance varies by context.
